PAC learning with stable and private predictions

We study binary classification algorithms for which the prediction on any point is not too sensitive to individual examples in the dataset. Specifically, we consider the notions of uniform stability (Bousquet and Elisseeff, 2001) and prediction privacy (Dwork and Feldman, 2018). Previous work on these notions shows how they can be achieved in the standard PAC model via simple aggregation of models trained on disjoint subsets of data. Unfortunately, this approach leads to a significant overhead in terms of sample complexity. Here we demonstrate several general approaches to stable and private prediction that either eliminate or significantly reduce the overhead. Specifically, we demonstrate that for any class $C$ of VC dimension $d$ there exists a $\gamma$-uniformly stable algorithm for learning $C$ with excess error $\alpha$ using $\tilde O(d/(\alpha\gamma) + d/\alpha^2)$ samples. We also show that this bound is nearly tight. For $\epsilon$-differentially private prediction we give two new algorithms: one using $\tilde O(d/(\alpha^2\epsilon))$ samples and another one using $\tilde O(d^2/(\alpha\epsilon) + d/\alpha^2)$ samples. The best previously known bounds for these problems are $O(d/(\alpha^2\gamma))$ and $O(d/(\alpha^3\epsilon))$, respectively.

==> privstab-realizable-lem.tex <==
\paragraph{Proof of Lemma~\ref{lem:realizable-alg}} \label{app:priv-real}

	Note that the proof uses the notations defined in Section~\ref{sec:pr-notations}.
	
	Let $N^{\mathrm{net}}_{\alpha,\beta,d}$ denote the minimal sample complexity required for Lemma~\ref{lem:eps-net-3} to hold, given parameters $\alpha, \beta$ and $d$.
	Assume that $m \ge r N^{\mathrm{net}}_{\alpha,\alpha,d}$,
	where $r = 3 \log (1/\epsilon)/\epsilon$, and we define a corresponding algorithm. Let $I_1,\dots, I_r$ be disjoint subsets of $[m]$ of size $N^{\mathrm{net}}_{\alpha,\alpha,d}$, drawn uniformly at random (namely, each $I_j$ is chosen uniformly at random from $[m] \setminus \left( \bigcup_{k=1}^{j-1} I_k \right)$). For any $j \in [r]$, let $h_{I_j} = \arg\min_{h \in H} L_{S_{I_j}}(h)$.
	Given any fixed $I_1,\dots,I_r$, define the hypothesis $h_{I_1,\dots,I_r}$ as follows, viewing it as a function from $X$ to $[0,1]$:
	\[
	h_{I_1,\dots,I_r}(x) = \frac{\exp\left(3 \log (1/\epsilon) \frac{1}{r}\sum_{j=1}^r h_{I_j}(x)\right)}{\exp\left(3 \log (1/\epsilon) \frac{1}{r}\sum_{j=1}^r h_{I_j}(x)\right) + \exp\left(3 \log (1/\epsilon) \frac{1}{r}\sum_{j=1}^r (1-h_{I_j}(x))\right)}.
	\]
	In other words, $h_{I_1,\dots,I_r}$ is a soft majority of $h_{I_1},\dots,h_{I_r}$. The final hypothesis is $\hat{h} = \E_{I_1 \cdots I_r} h_{I_1,\dots,I_r}$, namely, it equals $h_{I_1,\dots,I_r}$ when $I_1,\dots,I_r$ are randomly chosen.
	
	The algorithm is $O(\epsilon)$-private since by changing one point, one can change only one of the hypotheses $h_{I_j}$, and this changes the final hypothesis by at most a factor of $e^{O(\epsilon)}$. Next, assume that there exists $h^* \in H$ with $L_{S}(h^*) = 0$, and we will prove that $L_S(\hat{h}) \le O(\alpha)$. Let $\{Z_{j,i}\}_{j \in [r], i \in [m]}$ be an indicator of whether $h_{I_j}(x_i) \ne h^*(x_i)$, where $((x_i, h^*(x_i)))$ is the $i$'th example in the training set for $i \in [m]$. Since $|I_j| = N^{\mathrm{net}}_{\alpha,\alpha,d}$, with probability $1-\alpha$ it holds that $\sum_{i=1}^m Z_{j,i} \le \alpha m$. In particular, $\E_{I_1\cdots I_r} \sum_{j,i}[Z_{j,i}] \le 2\alpha m r$. Note that for any $i \in [m]$, if $\sum_j Z_{j,i} \le r/3$, then $|\tilde{h}(x_i) - h^*(x_i)| \le \alpha$. In particular,
	\[
	L_S(\hat{h})
	= \E_{I_1\cdots I_r} \left[\frac{1}{m} \sum_{i=1}^m |\tilde{h}(x_i) - h^*(x_i)|\right]
	\le \E_{I_1\cdots I_r} \left[\frac{1}{m} \sum_{i=1}^m \left(\alpha + \frac{3}{r} \sum_{j=1}^r Z_{j,i}\right) \right]
	\le 7 \alpha.
	\]
	
\yuval{end}


\begin{lemma}
	Assume that $m \ge 6 \eta m \log(1/\alpha) N^{\mathrm{net}}_{\alpha,\beta/r,d}$. Then, one can implement the private learner $\A^R_{1/\eta m, 4\alpha, \beta, d}$ such that with probability $1-\beta$ over $S$, for all $h \in H$, $\E_{(x,y)\sim D}[|h(x) - \A^R(S_h)(x)|] \le \alpha$.
\end{lemma}

\begin{proof}
	We will start by defining the transformation $h \mapsto \A^R(S_h)$: split the sample $S_h$ into $r = 6 \eta m \log(1/\alpha)$ partitions, each of size $N := N^{\mathrm{net}}_{\alpha,\beta,d}$, where partition $j$ contains examples $((x_i,h(x_i)))_{i=(j-1)N +1}^{j N}$. For any partition $j \in [r]$, the algorithm learns a hypothesis $\varphi_{S,j}(h)$: it is an arbitrary hypothesis with zero training loss on this partition. The final output $\varphi_S(h)$ is defined by
	\[
	\varphi_S(h) = \frac{\exp\left(\frac{\sum_{j=1}^r \varphi_{S,j}(h)}{2 \eta m}\right)}{\exp\left(\frac{\sum_{j=1}^r \varphi_{S,j}(h)}{2 \eta m}\right) + \exp\left(\frac{\sum_{j=1}^r (1-\varphi_{S,j}(h))}{2 \eta m}\right)},
	\]
	namely, a soft majority of the $\varphi_{S,j}$ functions. One can see that $\varphi_S(h)$ is $1/(\eta m)$ private with respect to $S_h$: changing one example can change only one of the hypotheses $h_j$ and this changes the prediction by at most $e^{1/\eta m}$ multiplicative factor.
	
	Next, we claim the following: fix $h \in H$ and assume that for all $j \in [r]$, $\E_{(x,y) \sim D}[|h(x) - \varphi_{S,j}(h)(x)|] \le \alpha$. Then, $\E_{(x,y) \sim D}[|h(x) - \varphi_S(x)|] \le 4\alpha$. Indeed, assume that this holds. One obtains that
	\[
	\E_{(x,y)\sim D}\left[\left|\frac{1}{r}\sum_{j=1}^r \varphi_{S,j}(h)(x) - h(x)\right|\right]
	\le \frac{1}{r} \sum_{j=1}^r \E_{(x,y)\sim D}\left[\left|\varphi_{S,j}(h)(x) - h(x)\right|\right]
	\le 4\alpha.
	\]
	By Markov's inequality,
	\begin{equation} \label{eq:223}
	\Pr_{(x,y)\sim D}\left[\left|\frac{1}{r}\sum_{j=1}^r \varphi_{S,j}(h)(x) - h(x)\right| > 1/3 \right] \le 3\alpha.
	\end{equation}
	Note that for any $x$ that satisfies $|\frac{1}{r}\sum_{j=1}^r \varphi_{S,j}(h)(x) - h(x)| \le 1/3$, $|\varphi_S(h)(x) - h(x)| \le \alpha$. Hence, by \eqref{eq:223}, one obtains that $\E_{(x,y) \sim D}[|h(x) - \varphi_S(h)(x)|] \le 4\alpha$, as required.
	
	It remains to show that with probability $1-\beta$, for all $j \in [r]$ and all $h \in H$, $\E_{(x,y) \sim D}[|h(x) - \varphi_{S,j}(h)(x)|] \le \alpha$. Indeed, this holds from the fact that with probability $1-\beta$, all partitions $S^{(j)}$ are $\alpha$-nets with respect to $D$. Note that $\varphi_{S,j}(h)$ agrees with $h$ on $S^{(j)}$, hence, if $S^{(j)}$ is an $\alpha$-net with respect to $D$, this implies that $\Pr_{(x,y) \sim D}[h(x) \ne \varphi_{S,j}(x)] \le \alpha$, as required.
\end{proof}

\begin{remark} \label{rem:1}
	Note that \eqref{eq:222} is stronger than Lemma~\ref{lem:realizable-alg}, and we will argue why it holds. We will first describe the realizable learner by \citet[Theorem~4.1]{DworkFeldman18} with privacy $\epsilon$ and accuracy $\alpha$, that given a training set $S$ output $\A(S)$:
	the training set is divided into $r = \tilde{\Theta}(\log(1/\alpha)/\epsilon)$ partitions $S^{(1)}, \dots, S^{(r)}$ of size $N^{\mathrm{net}}_{\alpha/4, \beta/r, d}$ each. From each partition $S^{(j)}$, the algorithm learns a hypothesis $\A(S,j) = \arg\min_{h \in H}L_{S^{(j)}}(h)$. The final hypothesis $\A(S)$ is a soft maximum of all predictors $\A(S,j)$ (in other words, $\A(S)$ is obtained via \emph{aggregation}). \citet{DworkFeldman18} show that this algorithm is $\epsilon$-private and $(\alpha,\beta)$-PAC, and we argue why \eqref{eq:222} holds as well.
	
	Switching back to the notation from our paper, recall that $\varphi_S(h) = \A(S_h)$ for $S_h = ((x_i, h(x_i)))_{i=1}^m$. 
	
	with probability $1-\beta$, all predictors $h_j$ have error $L_D(h_j) \le \alpha/4$.  \citet{DworkFeldman18} show that this implies that the output $\hat{h}$ has error  $L_D(\hat{h}) \le \alpha$. We argue that for any $h \in H$, and for any partition 
\end{remark}
